From modular forms to differential equations for Feynman integrals

In these proceedings we discuss a representation for modular forms that is more suitable for their application to the calculation of Feynman integrals in the context of iterated integrals and the differential equation method. In particular, we show that for every modular form we can find a representation in terms of powers of complete elliptic integrals of the first kind multiplied by algebraic functions. We illustrate this result on several examples. In particular, we show how to explicitly rewrite elliptic multiple zeta values as iterated integrals over powers of complete elliptic integrals and rational functions, and we discuss how to use our results in the context of the system of differential equations satisfied by the sunrise and kite integrals.

==> 2F1.tex <==
% !TEX root = ellipticproc.tex

\section{2F1}
\label{sec:2F1}

As an example of the ideas discussed in the previous sections, let us consider the family of integrals
\begin{align}
T(n_1,n_2,n_3) = \int_0^1 dx\, x^{-1/2 + n_1 + a\, \epsilon} (1-x)^{-1/2 + n_2 + b \epsilon} (1-z\, x)^{-1/2 + n_3 + c\,\epsilon}
\label{eq:2F1}
\end{align}
which is related to a special class of Hypergeometric functions and whose $\epsilon$-expansion 
has been studied in detail in ref.~\cite{Broedel:2017kkb}.
It is easy to show that all integrals in family~\eqref{eq:2F1}, for any choice of $n_1,n_2,n_3$, can be expressed as linear combination
of two independent master integrals, which can be chosen as
\begin{equation}
F_1 = T(0,0,0)\,, \quad F_2 = T(1,0,0)\,.
\end{equation} 
The two masters satisfy the system of two differential equations
\begin{align}
\partial_z\, F = (A + \epsilon B) F\,, \quad \mbox{with} \quad F = \left(  F_1 , F_2 \right)^T \label{eq:deqs2F1}
\end{align}
where $A,B$ are two $2 \times 2$ matrices
\begin{align}
A &= \frac{1}{z} \left( \begin{array}{ccc} 0 && 0 \\ 1/2 && -1 \end{array}  \right) + \frac{1}{z-1} \left( \begin{array}{ccc} -1/2 && 1/2 \\ -1/2 && 1/2  \end{array} \right) \\
B &= \frac{1}{z} \left( \begin{array}{ccc} 0 && 0 \\ a && -a-b  \end{array} \right) + \frac{1}{z-1} \left( \begin{array}{ccc} -a && a+b+c \\ -a && a+b+c  \end{array} \right)\,.
\end{align}
A suitable boundary condition for the differential equations~\eqref{eq:deqs2F1} can be determined by computing directly the integrals in Eq.~\eqref{eq:2F1} in $z=0$
\begin{align}
\lim_{z \to 0}F = \frac{\Gamma \left(a \epsilon +\frac{1}{2}\right) \Gamma \left(b \epsilon +\frac{1}{2}\right)}{\Gamma ( 1 + (a +b )\epsilon )}
\left( 1, \frac{2 a \epsilon +1}{2 \epsilon  (a+b)+2} \right)^T\,. \label{eq:bound}
\end{align}

We are now ready to solve the differential equations. 
It is relatively easy to see that by performing the following change of basis
\begin{align}
F = M G\,, \quad G = (G_1, G_2)^T
\end{align}
with
%\begin{align}
%M =\left(
%\begin{array}{cc}
% 2 K(z) & 0 \\
% \frac{\epsilon }{2 z (2 (a+b+c) \epsilon +1) K(z)}
% -\frac{2 E(z)}{z (2 (a+b+c) \epsilon +1)}
% +\frac{2 ((a+b) \epsilon +(a+c) z \epsilon +1) K(z)}{z (2 (a+b+c) \epsilon +1)} &
%   \frac{\epsilon }{2 z (2 (a+b+c) \epsilon +1) K(z)} 
%\end{array}
%\right)
%\end{align}
%
\begin{align}
M = \frac{1}{(2 (a+b+c) \epsilon +1)}\left(
\begin{array}{ccc}
 2 K(z) (2 (a+b+c) \epsilon +1) & & 0 \\ \\
 \frac{\epsilon }{2 z K(z)}
 -\frac{2 E(z)}{z }
 +\frac{2 ((a+b) \epsilon +(a+c) z \epsilon +1) K(z)}{z } & &
   \frac{\epsilon }{2 \,z \, K(z)} 
\end{array}
\right)\,,
\end{align}
the new master integrals $G_1,G_2$ fulfil the system of differential equations
\begin{align}
\partial_z G = \frac{\epsilon}{2\,z \, (z-1)\, K(z)^2}\, \Omega\, G \label{eq:neweq}
\end{align}
where the matrix $\Omega$ can be written as
\begin{align}
\Omega = \Omega_0 + \Omega_1 + \Omega_2
\end{align}
with
\begin{align}
&\Omega_0 = \frac{1}{4} \left(
\begin{array}{cc}
 1 & 1 \\
 -1 & -1 \\
\end{array}
\right) \,, \qquad 
\Omega_1 =  (a+b+(c-a) z) \, K(z)^2 \left(
\begin{array}{cc}
1 & 0 \\
 0 & 1 \\
\end{array}
\right)\,,\nonumber \\ 
&\Omega_2 = 4 \,  \left((a+b)^2+(a+c)^2 z^2-2 \left(a^2+b a+c a-b c\right) z\right) \, K(z)^4\, \left(
\begin{array}{cc}
 0 & 0 \\
 1 & 0 \\
\end{array}
\right)\,.
\end{align}
We stress that the differential equations in Eq.~\eqref{eq:neweq} are $\epsilon$-factorised.

In order to  \textsl{solve analytically} Eq.~\eqref{eq:neweq}, 
let us change variable from $z$ to the ratio of the periods $\tau$. Putting $z = \lambda(\tau) $, we find
$$\partial_z = \frac{\partial \tau}{\partial z} \partial_\tau = \frac{\pi \,i}{4 \lambda(\tau)(\lambda(\tau)-1) K(\lambda(\tau))^2}\, \partial_\tau$$
where we used the relation for the Haupmodul of $\Gamma(2)$,
$$ \quad 2 \pi \, i \partial_\tau \lambda(\tau) = 8 \lambda(\tau) (\lambda(\tau)-1) K(\lambda(\tau))^2\,. $$
In this way we find that the differential equations become
\begin{align}
\partial_\tau G = \frac{2\, \epsilon}{\pi \,i}\, \Omega\, G\,. \label{eq:neweq2}
\end{align}

As the last step, we know from the discussion in Section~\ref{sec:bla} 
 that a basis of modular forms of weight $2k$ for $\Gamma(2)$ is given by
$\lambda(\tau)^p K(\lambda(\tau))^{2 k}$, with $0\leq p \leq k$.
Using this, we see that the entries of $\Omega$ are indeed linear combinations of modular forms of $\Gamma(2)$, i.e.
we find explicitly

\begin{align}
K(\lambda(\tau))^2 &= - h_{2,1,0}^{(2)}(\tau) - \frac{1}{2} h_{2,1,1}^{(2)}(\tau) \nonumber \\
\lambda(\tau) K(\lambda(\tau))^2 &= - \frac{1}{2}h_{2,1,0}^{(2)}(\tau) -  h_{2,1,1}^{(2)}(\tau) \nonumber \\
K(\lambda(\tau))^4 &= - \frac{3}{2} h_{2,0,0}^{(4)}(\tau) + \frac{3}{2} h_{2,1,1}^{(4)}(\tau) \nonumber \\
\lambda(\tau) K(\lambda(\tau))^4 &=- \frac{3}{16} h_{2,0,0}^{(4)}(\tau) + \frac{3}{2} h_{2,1,0}^{(4)}(\tau)+ \frac{3}{2} h_{2,1,1}^{(4)}(\tau)\nonumber \\
\lambda(\tau)^2\, K(\lambda(\tau))^4 &= - \frac{3}{2} h_{2,0,0}^{(4)}(\tau) + \frac{3}{2} h_{2,1,0}^{(4)}(\tau)\,.
\end{align}
With this, and using the fact that the boundary condition in $z=0$, Eq.~\eqref{eq:bound}, translates directly into a boundary
condition in $\tau = i \infty$, we proved that the two entries of the vector $G$ can be written, to all orders in $\epsilon$,
in terms of iterated integrals of modular forms for $\Gamma(2)$.









